Eliminating Backdoor Triggers for Deep Neural Networks Using Attention Relation Graph Distillation

Due to the prosperity of Artificial Intelligence (AI) techniques, more and more backdoors are designed by adversaries to attack Deep Neural Networks (DNNs).Although the state-of-the-art method Neural Attention Distillation (NAD) can effectively erase backdoor triggers from DNNs, it still suffers from non-negligible Attack Success Rate (ASR) together with lowered classification ACCuracy (ACC), since NAD focuses on backdoor defense using attention features (i.e., attention maps) of the same order. In this paper, we introduce a novel backdoor defense framework named Attention Relation Graph Distillation (ARGD), which fully explores the correlation among attention features with different orders using our proposed Attention Relation Graphs (ARGs). Based on the alignment of ARGs between both teacher and student models during knowledge distillation, ARGD can eradicate more backdoor triggers than NAD. Comprehensive experimental results show that, against six latest backdoor attacks, ARGD outperforms NAD by up to 94.85% reduction in ASR, while ACC can be improved by up to 3.23%.

==> approach.tex <==
\section{Approach}
\label{sec:intro}
%1：提出角度 我们方法提出通过模型特征图之间的区别，获取模型与后门之间的关系。
%防御设置：
%本文所提出防御方法主要集中于人工智能场景中，即为在消除后门攻击的同时，尽可能小的影响模型在干净数据集上的性能。
%贡献：1. 

%2、为什么这样做？现有方法存在的问题？你这么做的原因？
%现有方法存在问题的原因：现今为止多数方法只考虑后门模型与干净模型相同非线性层之间的差别，希望通过后门模型与干净模型之间的特征图逼近获取干净数据。但是，由于高阶特征是由低阶特征经过非线性变幻得到的，现今方法没有考虑不同阶数的特征之间的关系，例如低阶特征转换成为高阶特征的转换关系，这却是后门攻击所产生的原因。获取转换关系损失，即为转换方法的损失。

%我们的核心想法是启发于ICML2021这篇文章的启发，文中提出对于特征，不同阶段的图像特征对于网络分类的，浅层网络所学习到的特征由于过于简单，往往更加容易受到后门攻击的影响，而深层网络所学习到的特征通常是复杂程度不同的的特征，高层次特征是通过低层次特征经过模型编码处理所得到的，高层特征往往更加的稳定，可是也丢失了图片的低阶特征，往往只使用高阶特征虽然会提高模型的鲁棒性，但是并不会提高模型的性能。
%到目前为止，有些方法虽然通过注意力机制等转移方式，将携带后门的模型进行了后门擦除，但是这一方法并未考虑不同阶数特征的关系，只是相当于另一个特征的处理过程，本文提出使用特征联系图损耗，通过寻找每层特征的损耗趋势与关系，利用极少的特征图片高效的修复模型中的后门漏洞并消除后门攻击对于模型的影响。


In this section, we first introduce the difference between the tradition fine-tune framework and our FRD framework. We then introduce the 
The core idea is inspired by \cite{ICML2021} which proposed that image features at different orders are for network classification. 
After the backdoor model is trained on a large number of data sets, it will gradually move closer to the clean model, which is also the most intuitive way of erasing backdoor features. However, in actual situations, due to the unequal number of data samples, the number of clean data samples only occupies a very small amount required for model training, so this method cannot effectively erase the existence of backdoor attacks.
To apply the relationship between different order features into the distillation  process of backdoor attack defence, we measure the features of different order in the model with different distance, and establish a deep relation graph  both inside teacher and student models based on the different order features. 
The relation graph exploits the knowledge structure loopholes inside backdoor network and can be regarded as a new defense mode in the artificial intelligence safety.
Distilling the feature components relation graph for backdoor enables not only sufficient knowledge passing but also transfer the clean knowledge graph of the different order feature embedding.
We focuses on efficiently removing the impact of backdoor attacks for the backdoor model, while affecting the accuracy of the model on the clean data set as little as possible. 

So far, most methods only consider the difference between the same nonlinear layer of the backdoor model and the clean model, and hope to obtain clean data through the feature map approximation between the backdoor model and the clean model. 
However, because high-order features are obtained from low-order features through non-linear layer changes, current methods do not consider the relationship between features of different orders. 
Thus, it is reasonable to consider the backdoor attack is change the relation graph inside the model. Next, we will introduce the feature relation graph between different order features and the graph distillation loss modeling process.

\subsection{Feature Attention Relation Graph}
%为了将不同阶数特征之间的关系用于后门攻击的蒸馏擦拭,我们将模型中不同阶数的特征进行不同距离的度量，建立不同特征中损耗图结构模型。我们采用的特征关系图架构如图1所示.
%由于不同阶数特征之间的损耗关系与联系程度不同，我们提出使用三个不同的特征表示后门模型与传统干净模型之间的蒸馏表示关系。
%我们所提出的关系图结构并不同于文章21中所提出的关系图结构关系，首先Li所提出的图结构关系是作用于图像的识别准确率，其次文章所提出的图结构关系并不同于之前的结构，之前结构中其点为图像不同批次的像素块，并非带有后门的注意力结构像素图。
%1.点的距离：我们将后门模型与教师模型之间的特征图直接建立距离损失关系，这是最直观的能表示后门模型与干净模型表示关系，如果在大量数据集训练中，后门模型将会逐渐接近干净模型，这也是最能想到的同阶特征关系表示方式转移。

To apply the relationship between different order feature components into the distillation  process of backdoor attack defence, we measure the feature components of different order in the model with different distance, and establish the feature component relation graph  distillation model of different order features. We proposed distillation architecture as followed as figure 1 (c). 
In feature component relation graph, each node represents one order feature component for an image, which is corresponded to a layer encoding in the knowledge structure of the model. The edge represents the semantic relationship between two nodes, which also exposes the knowledge structure representation in the feature component of two different orders in the backdoor attack model.

The structure of the  graph we proposed is different from the feature component relation graph proposed in Article 21. 
First, the graph structure relationship proposed by Li acts on the regression accuracy of the image patch, and secondly, our graph structure relationship proposed in the article is different from the previous structure. The nodes in the previous structure are pixel blocks of different batches of the image, not a map of the attention structure with the backdoor vulnerability. That's why it is reasonable to model relations between different order feature  than independent pixels.
We used the different order features to transfer knowledge system of the neural network model.  %CVPR21 and ICML.

The strong relation between different order features transferred from teacher to student would serve for defencing backdoor attack in our method. Based on the loss relationship and connection degree between different order features are different, we propose to use three different features to represent the distillation relationship between the backdoor model and the traditional clean model.

Note that we used the same order feature inside clean and backdoor model to build the feature relation graph. For the clean and backdoor model, the feature component relation graph is modelled as $G=(\mathbb{N}, \varepsilon)$, where $\mathbb{N}$ represents the node sets of the relation graph, $\varepsilon$ denotes the edge set of the relation graph. The following subsection will introduce
 the define of node and edge in feature relation graph.
 

%2： 特征图节点距离
\subsubsection{Nodes}
%后门模型在大量数据集上训练后，会逐渐向clean模型靠拢，这也是最直观的后门特征抹去方式。然而，在实际情况下，由于数据样本存在的数量不对等特性，干净数据样本的数量只占有模型训练所需数量极少数，所以这种方式并不能高效的抹去后门攻击的存在。不同于之前的关系图特征，我们采用相同阶数特征的注意力图作为点的特征，通过针对每层的注意力特征与最终的逻辑结果作为当前的模型输出的点特征。
Different from the previous relationship graph features, we found that the attention mechanism is very effective in the defense of backdoor attacks. In addition, the attention feature of different layers also have certain correlations. Therefore, it is reasonable to use the correlation of the attention mechanism between different layers to defend against backdoor attacks. 

When building the graph model, we directly use the attention features of the multi-level order features as the nodes in our feature  attention relation graph. First, we construct nodes based  on the attention features of the DNN model. 
The attention maps  are considered as an embedding vector in each order features, which can be represented as the knowledge node in the feature relation graph. 
The final logical result of teacher model and student model as the finally node   in the feature attention relation graph. 
Given a DNN model $M$, we define the $p$-$th$ order feature map  as $F^{p} = M^{p}(X)$ which is build as a  vector of three dimensions (channel, width, height) for input image $X$. 
The attention extraction operation is defined as $T^{p} = \Lambda (F^{p})$, where $T^{p}$ represents the $p$-$th$ order attention map extract from the $F^{p}$ .

The attention extract function is defined as follow as
\begin{equation}
\Lambda (F^{p}(X)) = \frac{1}{C}\sum_{i=1}^{C} \left | F^{p}_{i}(X) \right |^{2},
\label{node_distance}
\end{equation}
where $C$ is the feature dimension of the channel, $\left | \cdot  \right |$ is the the absolute value function.
Based on the attention extract function, the $p$-$th$ order feature can be transformed as the attention feature in the relation graph for the node. Then, the node set in $G$ are denoted as $\mathbb{N} = \left \{ T^{1}_{M}, T^{2}_{M}, ..., T^{p}_{M},..., L_{M}\right \}$, where $L_{M}$ is the logits  of the DNN model $M$ for the image $X$.

%点的距离也就是最初的特征图像素之间的差距计算损失，我们直接将老师与学生模型中相同阶数的特征图像进行提取，将

%3 特征关系边的距离
\subsubsection{Edges}
%
As shown in the Fig1, the edge set in $G$ is represented as the relation between attention features of different orders, which is defined as $\varepsilon = \left \{E_{i j}\right \}^{k\times k}$, where $k+1$ is the size of  node set. In our  attention relation graph, each attention node is connected by an edge, except for the last logits node. $E_{i j}$ denotes the the Euclidean distance between the instance features of two linked instances of the $i-th$ and the $j-th$ nodes in the same model, which also means  the similarity  connection between the $i$-$th$ and the $j$-$th$ node. The edge function can be expressed as 
\begin{equation}
E(T_{i}, T_{j}) = Similarity(trans(T_{i}), trans(T_{j})),
\label{edge_distance}
\end{equation}
where the $similarity$ is the squared difference function for the sample of attention features.
To calculating the Euclidean distance to the different order attention, the $trans$ function can change the attention tensor to the same dimensions.
Based on the edge function, the changes of the attention features of each layer will be stored in the adjacency matrix $A$ of the attention relation graph that we defined in the form of instance $p$-$th$ attention similarity.
%当注意力关系图中的点与边都定义完成后，这张注意力关系图就能代表模型的各层注意力特征知识体系。

\subsection{Attention Graph Distillation Loss }
When the nodes and edges in the attention graph are defined, the attention graph can represent the attention feature knowledge system of the model. 
Article X proves that the backdoor attack mainly changes the attention mechanism in the feature map, making the model pay more attention to the connection between the backdoor feature and the instance. Therefore, we use the attention graph transformation method to eliminate the influence of backdoor features on the model. Our attention graph distillation  loss $\mathfrak{L}_{G}$ is defined as follow as
\begin{equation}
    \mathfrak{L}_{G}\left ( G_{S}, G_{\mathbb{C}} \right )= \lambda _{n}\cdot\mathfrak{L}_{\mathbb{N}}+ \lambda _{e}\cdot\mathfrak{L}_{\varepsilon},
\end{equation}
where $\lambda_{n}$ and $\lambda_{e}$ is the hyper-parameter for balanced the contribution ratio of node and edge between backdoor model $S$ and the clean teacher model $\mathbb{C}$.
The node loss function is defined as follow as 
\begin{equation}
    \mathfrak{L}_{N}\left ( \mathbb{N}_{S}, \mathbb{N}_{\mathbb{C}} \right ) = \frac{1}{k} \sum_{i=0}^{k}\lambda _{i}\cdot {\left \| \frac{T_{\mathbb{C}}^{i}}{\left \|T_{\mathbb{C}}^{i} \right \|_{2}} - \frac{T_{S}^{i}}{\left \|T_{S}^{i} \right \|_{2}} \right \|_{2}},
    \label{node_loss}
\end{equation}

where the $\left \| \cdot  \right \|_{2}$ is the $L_{2}$ norm operation and $\lambda$ is the  percentage of each order attention in the node loss which represents the contribution of  different order attention features in node loss function.

The edge loss function is defined as follow as 
\begin{equation}
    \mathfrak{L}_{\varepsilon}\left ( E_{S}, E_{\mathbb{C}} \right )= \frac{1}{k}\sum_{i=1}^{k}\sum_{j=1}^{k}\left \|E_{\mathbb{C}}^{ij} - E_{S}^{ij}  \right \|_{2}^{2}.
\end{equation}




\subsection{Overall Loss }
%不同于传统的知识蒸馏机制，在我们关系图机制中，整体的损失由三种不同的损失函数进行计算
Different from the traditional knowledge distillation mechanism, the overall loss of our attention relation graph for backdoor model is calculated by three different loss functions, which is defined as follow as 
\begin{equation}
    \mathfrak{L}_{all}= \mathfrak{L}_{G}+\mathfrak{L}_{logits}+\mathfrak{L}_{CE}.
\end{equation}
where the $\mathfrak{L}_{logits}$ is the traditional knowledge distillation logits loss for clean model, and the $\mathfrak{L}_{CE}$ is the cross entropy loss to target.




==> experiment.tex <==
\section{Experiment}
\label{sec:exp}
To evaluate the effectiveness of our  framework, we
implemented FAGD based on  Pytorch (version 1.4.0). 



RQ1: 

\subsection{Experiment Setting}



==> introduction.tex <==
\section{Introduction}
\label{sec:intro}
So far, most methods only consider the difference between the same nonlinear layer of the backdoor model and the clean model and hope to obtain clean data through the feature map approximation between the backdoor model and the clean model. 
However, because high-order features are obtained from low-order features through non-linear layer changes, current methods do not consider the relationship between features of different orders. For example, the conversion relationship between low-order features into high-order features is a backdoor attack.


% Our method proposes to obtain the relationship between the model and the backdoor through the difference between the model feature maps.
% The method in this paper mainly focuses on eliminating the backdoor attack while affecting the accuracy of the current model as little as possible, and even improving the accuracy of the model under better circumstances.
% So far, although some methods transfer non-robust features in backdoor attacks through transfer methods such as attention Characteristics of the attrition trend, to find out the loophol，es in the backdoor attack.

To address the issue, we proposed a backdoor feature relation graph distillation erase method, which is inspired by the ICML2021 article which proposed that image features at different stages are for network classification. 
% The features learned by shallow layer networks are often more susceptible to backdoor attacks because they are too simple. The features learned by the deep network are usually features with different levels of complexity. High-level features are obtained through model coding through low-level features. High-level features are often more stable, but the low-level features of the picture are  lost. 
% Often only using the same order features will improve the robustness of the model in a limited extent, but it will not improve the performance of the model.
So far, although some methods have used the attention mechanism and other transfer methods to defence the model carrying the backdoor, this method does not consider the relationship between the features of different orders, but is equivalent to the processing process of another feature In this paper, we propose to use the loss of feature connection graphs to find the loss trend and relationship of each layer of features, and use very few feature images to efficiently repair the backdoor vulnerabilities in the model and eliminate the impact of backdoor attacks on the model. 

==> ref.tex <==
\begin{thebibliography}{20}\itemsep=-1pt

\bibitem{Adi2018TurningYW}
Yossi Adi, Carsten Baum, Moustapha Ciss{\'e}, Benny Pinkas, and Joseph Keshet.
\newblock Turning your weakness into a strength: Watermarking deep neural   networks by backdooring.
\newblock In {\em USENIX Security Symposium}, 2018.

\bibitem{backdoor-federated}
Eugene Bagdasaryan, Andreas Veit, Yiqing Hua, Deborah Estrin, and Vitaly  Shmatikov.
\newblock How to backdoor federated learning.
\newblock In {\em International Conference on Artificial Intelligence and   Statistics}, pages 2938--2948, 2020.

\bibitem{backdoor-detect}
Nathalie Baracaldo Heiko Ludwig Benjamin Edwards Taesung Lee Ian~Molloy
  Bryant~Chen, Wilka~Carvalho and Biplav Srivastava.
\newblock Detecting backdoor attacks on deep neural networks by activation
  clustering.
\newblock In {\em AAAI Workshop}, pages 39--57, 2019.

\bibitem{evaluation}
Nicholas Carlini and David Wagner.
\newblock Towards evaluating the robustness of neural networks.
\newblock In {\em IEEE Symposium on Security and Privacy (SP)}, pages 39--57,
  2017.

\bibitem{blend}
Xinyun Chen, Chang Liu, Bo Li, Kimberly Lu, and Dawn Song.
\newblock Targeted backdoor attacks on deep learning systems using data
  poisoning.
\newblock {\em arXiv preprint arXiv:1712.05526}, 2017.

\bibitem{Chou2020SentiNetDL}
Edward Chou, Florian Tram{\`e}r, and Giancarlo Pellegrino.
\newblock Sentinet: Detecting localized universal attacks against deep learning   systems.
\newblock {\em IEEE Security and Privacy Workshops (SPW)}, pages 48--54, 2020.

\bibitem{adversarial}
Ian~J Goodfellow, Jonathon Shlens, and Christian Szegedy.
\newblock Explaining and harnessing adversarial examples.
\newblock In {\em ICLR}, 2014.

\bibitem{badnets}
Tianyu Gu, Kang Liu, Brendan Dolan-Gavitt, and Siddharth Garg.
\newblock Badnets: Evaluating backdooring attacks on deep neural networks.
\newblock {\em IEEE Access}, 7:47230--47244, 2019.

\bibitem{resnet}
Kaiming He, Xiangyu Zhang, Shaoqing Ren, and Jian Sun.
\newblock Deep residual learning for image recognition.
\newblock In {\em CVPR}, pages 770--778, 2016.

\bibitem{Kolouri_detection_based}
Soheil Kolouri, Aniruddha Saha, Hamed Pirsiavash, and Heiko Hoffmann.
\newblock Universal litmus patterns: Revealing backdoor attacks in cnns.
\newblock In {\em CVPR}, June 2020.

\bibitem{komodakis2017paying}
Nikos Komodakis and Sergey Zagoruyko.
\newblock Paying more attention to attention: improving the performance of
  convolutional neural networks via attention transfer.
\newblock In {\em ICLR}, 2017.

\bibitem{NAD}
Yige Li, Xixiang Lyu, Nodens Koren, Lingjuan Lyu, Bo Li, and Xingjun Ma.
\newblock Neural attention distillation: Erasing backdoor triggers from deep
  neural networks.
\newblock In {\em ICLR}, 2020.

\bibitem{Li2020RethinkingTT}
Yiming Li, Tongqing Zhai, Baoyuan Wu, Yong Jiang, Zhifeng Li, and Shutao Xia.
\newblock Rethinking the trigger of backdoor attack.
\newblock {\em ArXiv}, abs/2004.04692, 2020.

\bibitem{Liu2021RemovingBW}
Xuankai Liu, Fengting Li, Bihan Wen, and Qi Li.
\newblock Removing backdoor-based watermarks in neural networks with limited
  data.
\newblock {\em International Conference on Pattern Recognition (ICPR)}, pages
  10149--10156, 2021.

\bibitem{liu2019knowledge}
Yufan Liu, Jiajiong Cao, Bing Li, Chunfeng Yuan, Weiming Hu, Yangxi Li, and
  Yunqiang Duan.
\newblock Knowledge distillation via instance relationship graph.
\newblock In {\em CVPR}, pages 7096--7104, 2019.

\bibitem{trojan}
Yingqi Liu, Shiqing Ma, Yousra Aafer, Wen-Chuan Lee, Juan Zhai, Weihang Wang,
  and Xiangyu Zhang.
\newblock Trojaning attack on neural networks.
\newblock In {\em Network and Distributed Systems Security (NDSS)}, 2017.





\bibitem{liu2020reflection}
Yunfei Liu, Xingjun Ma, James Bailey, and Feng Lu.
\newblock Reflection backdoor: A natural backdoor attack on deep neural
  networks.
\newblock In {\em ECCV}, pages 182--199, 2020.

\bibitem{cleanlabel}
Rui Ning, Jiang Li, Chunsheng Xin, and Hongyi Wu.
\newblock Invisible poison: A blackbox clean label backdoor attack to deep
  neural networks.
\newblock In {\em INFOCOM}, pages 1--10, 2021.

\bibitem{papernot2016distillation}
Nicolas Papernot, Patrick McDaniel, Xi Wu, Somesh Jha, and Ananthram Swami.
\newblock Distillation as a defense to adversarial perturbations against deep
  neural networks.
\newblock In {\em IEEE Symposium on Security and Privacy (SP)}, pages 582--597.
  IEEE, 2016.

\bibitem{interpreting}
Jie Ren, Mingjie Li, Zexu Liu, and Quanshi Zhang.
\newblock Interpreting and disentangling feature components of various
  complexity from dnns.
\newblock In {\em ICML}, 2021.

\bibitem{Shafahi2018PoisonFT}
Ali Shafahi, W.~Ronny Huang, Mahyar Najibi, Octavian Suciu, Christoph Studer,
  Tudor Dumitras, and Tom Goldstein.
\newblock Poison frogs! targeted clean-label poisoning attacks on neural
  networks.
\newblock In {\em NeurIPS}, 2018.

\bibitem{Song2021FDA3FD}
Yunfei Song, Tian Liu, Tongquan Wei, Xiangfeng Wang, Zhe Tao, and Mingsong
  Chen.
\newblock {FDA$^3$} : Federated defense against adversarial attacks for
  cloud-based iiot applications.
\newblock {\em IEEE Transactions on Industrial Informatics}, 17:7830--7838,
  2021.

\bibitem{sig}
Brandon Tran, Jerry Li, and Aleksander Madry.
\newblock Spectral signatures in backdoor attacks.
\newblock In {\em NeurIPS}, 2018.

\bibitem{truong2020systematic}
Loc Truong, Chace Jones, Brian Hutchinson, Andrew August, Brenda Praggastis,
  Robert Jasper, Nicole Nichols, and Aaron Tuor.
\newblock Systematic evaluation of backdoor data poisoning attacks on image
  classifiers.
\newblock In {\em CVPR}, pages 788--789, 2020.

\bibitem{neuralclean}
Bolun Wang, Yuanshun Yao, Shawn Shan, Huiying Li, Bimal Viswanath, Haitao
  Zheng, and Ben~Y Zhao.
\newblock Neural cleanse: Identifying and mitigating backdoor attacks in neural
  networks.
\newblock In {\em IEEE Symposium on Security and Privacy (SP)}, pages 707--723,
  2019.

\bibitem{wang2019convergence}
Yisen Wang, Xingjun Ma, James Bailey, Jinfeng Yi, Bowen Zhou, and Quanquan Gu.
\newblock On the convergence and robustness of adversarial training.
\newblock In {\em ICML}, volume~1, page~2, 2019.

\bibitem{Wang2020ImprovingAR}
Yisen Wang, Difan Zou, Jinfeng Yi, James Bailey, Xingjun Ma, and Quanquan Gu.
\newblock Improving adversarial robustness requires revisiting misclassified
  examples.
\newblock In {\em ICLR}, 2020.

\bibitem{Backdoor_phy}
Emily Wenger, Josephine Passananti, Arjun~Nitin Bhagoji, Yuanshun Yao, Haitao
  Zheng, and Ben~Y. Zhao.
\newblock Backdoor attacks against deep learning systems in the physical world.
\newblock In {\em CVPR}, pages 6206--6215, June 2021.

\bibitem{Xie2020DBADB}
Chulin Xie, Keli Huang, Pin-Yu Chen, and Bo Li.
\newblock Dba: Distributed backdoor attacks against federated learning.
\newblock In {\em ICLR}, 2020.

\bibitem{MCR}
Pu Zhao, Pin-Yu Chen, Payel Das, Karthikeyan~Natesan Ramamurthy, and Xue Lin.
\newblock Bridging mode connectivity in loss landscapes and adversarial
  robustness.
\newblock {\em ICLR}, 2020.

\end{thebibliography}

==> reference.tex <==


\bibitem{adversarial}
{Ian J Goodfellow, Jonathon Shlens, and Christian Szegedy,}
Explaining and harnessing adversarial
examples.
In \emph{Proc. of ICLR},  2014.


\bibitem{Deepinspect}
{Huili Chen, Cheng Fu, Jishen Zhao, and Farinaz Koushanfar,}
 Deepinspect: A black-box trojan
detection and mitigation framework for deep neural networks.
In \emph{Proc. of IJCAI},  2019.


\bibitem{backdoor-detect}
{Bryant Chen, Wilka Carvalho, Nathalie Baracaldo, Heiko Ludwig, Benjamin Edwards, Taesung
Lee, Ian Molloy, and Biplav Srivastava.}
 Detecting backdoor attacks on deep neural networks by
activation clustering.
In \emph{Proc. of AAAI Workshop},  2019.
% Ian J Goodfellow, Jonathon Shlens, and Christian Szegedy. Explaining and harnessing adversarial
% examples. In ICLR, 2014.

% Huili Chen, Cheng Fu, Jishen Zhao, and Farinaz Koushanfar. Deepinspect: A black-box trojan
% detection and mitigation framework for deep neural networks. In IJCAI, 2019b.



% Bryant Chen, Wilka Carvalho, Nathalie Baracaldo, Heiko Ludwig, Benjamin Edwards, Taesung
% Lee, Ian Molloy, and Biplav Srivastava. Detecting backdoor attacks on deep neural networks by
% activation clustering. In AAAI Workshop, 2019a


\bibitem{evaluation}
{Nicholas Carlini and David Wagner.}
 Towards evaluating the robustness of neural networks. 
In \emph{Proc. of SP},  2017.
% Nicholas Carlini and David Wagner. Towards evaluating the robustness of neural networks. In SP,
% 2017

\bibitem{backdoor-federated}
{Eugene Bagdasaryan, Andreas Veit, Yiqing Hua, Deborah Estrin, and Vitaly Shmatikov..}
 How to
backdoor federated learning.
In \emph{Proc. of AISTATS},  2020.
% Eugene Bagdasaryan, Andreas Veit, Yiqing Hua, Deborah Estrin, and Vitaly Shmatikov. How to
% backdoor federated learning. In AISTATS, 2020

\bibitem{backdoor-federated}
{Yiming Li, Baoyuan Wu, Yong Jiang, Zhifeng Li, and Shu-Tao Xia.}
Backdoor learning: A survey.
In \emph{arXiv preprint arXiv:2007.08745},  2020.

% Yiming Li, Baoyuan Wu, Yong Jiang, Zhifeng Li, and Shu-Tao Xia. Backdoor learning:arXiv preprint arXiv:2007.08745 A survey.
% arXiv preprint arXiv:2007.08745, 2020a

% Yiming Li, Tongqing Zhai, Baoyuan Wu, Yong Jiang, Zhifeng Li, and Shutao Xia. Rethinking the
% trigger of backdoor attack.

\bibitem{backdoor-reflection}
{Yunfei Liu, Xingjun Ma, James Bailey, and Feng Lu.}
Reflection backdoor: A natural backdoor
attack on deep neural networks.
In \emph{Proc. of ECCV},  2020.


% Yunfei Liu, Xingjun Ma, James Bailey, and Feng Lu. Reflection backdoor: A natural backdoor
% attack on deep neural networks. In ECCV, 2020b

\bibitem{backdoor-federated}
{Yunfei Liu, Xingjun Ma, James Bailey, and Feng Lu.}
Reflection backdoor: A natural backdoor
attack on deep neural networks.
In \emph{Proc. of ECCV},  2020.


Yingqi Liu, Shiqing Ma, Yousra Aafer, Wen-Chuan Lee, Juan Zhai, Weihang Wang, and Xiangyu
Zhang. Trojaning attack on neural networks

% Aleksander Madry, Aleksandar Makelov, Ludwig Schmidt, Dimitris Tsipras, and Adrian Vladu.
% Towards deep learning models resistant to adversarial attacks. In ICLR, 2018.

Nicolas Papernot, Patrick McDaniel, Xi Wu, Somesh Jha, and Ananthram Swami. Distillation as a
defense to adversarial perturbations against deep neural networks. In S&P. IEEE, 2016.

Ali Shafahi, W Ronny Huang, Mahyar Najibi, Octavian Suciu, Christoph Studer, Tudor Dumitras,
and Tom Goldstein. Poison frogs! targeted clean-label poisoning attacks on neural networks. In
NeurIPS, 2018

Brandon Tran, Jerry Li, and Aleksander Madry. Spectral signatures in backdoor attacks. In NeurIPS,
2018

% Loc Truong, Chace Jones, Brian Hutchinson, Andrew August, Brenda Praggastis, Robert Jasper,
% Nicole Nichols, and Aaron Tuor. Systematic evaluation of backdoor data poisoning attacks on
% image classifiers. In CVPR, 2020.

Alexander Turner, Dimitris Tsipras, and Aleksander Madry. Clean-label backdoor attacks.
https://people.csail.mit.edu/madry/lab/, 2019.

Yisen Wang, Xingjun Ma, James Bailey, Jinfeng Yi, Bowen Zhou, and Quanquan Gu. On the
convergence and robustness of adversarial training. In ICML, 2019b.

Bolun Wang, Yuanshun Yao, Shawn Shan, Huiying Li, Bimal Viswanath, Haitao Zheng, and Ben Y
Zhao. Neural cleanse: Identifying and mitigating backdoor attacks in neural networks. In S&P.
IEEE, 2019a

Sergey Zagoruyko and Nikos Komodakis. Paying more attention to attention: Improving the performance of convolutional neural networks via attention transfer. In ICLR, 2017.
Hongyi Zhang, Moustapha Cisse, Yann N Dauphin, and David Lopez-Paz. mixup: Beyond empirical


Pu Zhao, Pin-Yu Chen, Payel Das, Karthikeyan Natesan Ramamurthy, and Xue Lin. Bridging mode
connectivity in loss landscapes and adversarial robustness. In ICLR, 2020a.



Kaiming He, Xiangyu Zhang, Shaoqing Ren, and Jian Sun. Deep residual learning for image recognition. In CVPR, 2016.
